Predicting User Knowledge Gain in Informational Search Sessions

Web search is frequently used by people to acquire new knowledge and to satisfy learning-related objectives. In this context, informational search missions with an intention to obtain knowledge pertaining to a topic are prominent. The importance of learning as an outcome of web search has been recognized. Yet, there is a lack of understanding of the impact of web search on a user's knowledge state. Predicting the knowledge gain of users can be an important step forward if web search engines that are currently optimized for relevance can be molded to serve learning outcomes. In this paper, we introduce a supervised model to predict a user's knowledge state and knowledge gain from features captured during the search sessions. To measure and predict the knowledge gain of users in informational search sessions, we recruited 468 distinct users using crowdsourcing and orchestrated real-world search sessions spanning 11 different topics and information needs. By using scientifically formulated knowledge tests, we calibrated the knowledge of users before and after their search sessions, quantifying their knowledge gain. Our supervised models utilise and derive a comprehensive set of features from the current state of the art and compare performance of a range of feature sets and feature selection strategies. Through our results, we demonstrate the ability to predict and classify the knowledge state and gain using features obtained during search sessions, exhibiting superior performance to an existing baseline in the knowledge state prediction task.

==> backup.tex <==
\section{tables}

%this is the table of features, wsdm version, feature named with numbers

\begin{table}[h]
\centering
\caption{\small{Features for supervised prediction of knowledge gain.}}
\ran{might need a better approach for the categorization of the features - e.g. Session including the other categories, some are hard to decide which category it belongs to}
%\scalebox{0.75}{
\begin{adjustbox}{max width=0.5\textwidth}
\small
\begin{tabular}{ p{1cm} p{1.4cm} p{7cm} }
\toprule
\textbf{Category} & \textbf{Notation} & \textbf{Feature description}\\ 

\midrule

\multirow{1}{*}{\emph{Session}} & $t^{s}_{1}$ & Session duration \\
%& $t^{s}_{2}$ & Average duration per query\\
%& & \\
\midrule

\multirow{11}{*}{\emph{Query}} & $t^{q}_{1}$ & Number of queries in session $s$ \\[0.02cm]
& $t^{q}_{2},t^{q}_{3},t^{q}_{4}$ & Maximum, minimum, average number of query terms \\[0.02cm]
& $t^{q}_{5},t^{q}_{6},t^{q}_{7}$ & Maximum, minimum, average number of uniq terms per query \\[0.02cm]
& $t^{q}_{8}$ & Total number of query terms \\[0.02cm]
& $t^{q}_{9}$ & Total number of uniq terms in all queries \\[0.02cm]
& $t^{q}_{10}$ & Number of query terms / unique query terms ($\frac {t^{q}_{8}}{t^{q}_{9}}$) \\[0.02cm]
& $t^{q}_{11}, t^{q}_{12}$ & First, last query length \\[0.02cm]
& $t^{q}_{13}, t^{q}_{14}$ & First, last query uniq terms \\[0.02cm]
%& $t^{q}_{14}$ & Avg time interval between queries \\[0.02cm]
%& $t^{q}_{15}$ & Total time spent on landing pages \\[0.02cm]
%& $t^{q}_{16}$ & Average time spent on a landing page per query \\[0.02cm]
\midrule
\multirow{12}{*}{\emph{SERP Click}}& $t^{c}_{1}$ &  Total number of click \\[0.02cm]

&$t^{c}_{2}, t^{c}_{3}, t^{c}_{4}$ & Average, highest, lowest rank of the clicks \\[0.02cm]
 & $t^{c}_{5}$ & Average interval between clicks\\[0.02cm]
 & $t^{c}_{6}$ & Average number of clicks per query\\[0.02cm]
%  &$t^{c}_{7} $& Average time between a query and the first click\\[0.02cm]
   &$t^{c}_{7}, t^{c}_{8}$& Number, percentage of queries with no clicks \\ [0.02cm]
\midrule
\multirow{10}{*}{\emph{Browsing}} & $t^{b}_{1}$ & Number of pages viewed\\[0.02cm]
  & $t^{b}_{2} $ & Average number of page viewed per query \\[0.02cm]
   & $t^{b}_{3}$ & Number of uniq pages viewed \\[0.02cm]
   & $t^{b}_{4} $ & Average number of uniq page viewed per query \\[0.02cm]
 & $t^{b}_{5}$ & Total stay time on the pages \\[0.02cm]
  & $t^{b}_{6}$ & Average stay time on the pages per query \\[0.02cm]
 & $t^{b}_{7}, t^{b}_{8}$ & Maxium, average stay time on the pages \\[0.02cm]
  & $t^{b}_{9}$ & Total active time on the pages \\[0.02cm]
  & $t^{b}_{10}, t^{b}_{11}$ & Maximum, average active time on the pages per query \\[0.02cm]
 & $t^{b}_{12}, t^{b}_{13}$ & Maxium, average active time on the pages \\[0.02cm]
  & $t^{b}_{14}, t^{b}_{15},t^{b}_{16}$ & Total, average, maximum stay time on SERPs \\[0.02cm]
  & $t^{b}_{17}, t^{b}_{18},t^{b}_{19}$ & Total, average, maximum active time on SERPs \\[0.02cm]
  & $t^{b}_{20} $ & Ratio of revisited pages \\[0.02cm]
  & $t^{b}_{21},t^{b}_{22} $ & Number, percentage of pages visited through SERP \\[0.02cm]
  & $t^{b}_{23},t^{b}_{24} $ & Number, percentage of pages visited through SERP \\[0.02cm]
 &$t^{b}_{25} $  & total number of mouseovers in the session. \\
&$t^{b}_{26} $  & average number of mouseovers per query. \\
&$t^{b}_{27} $  & max mouseover rank in the session. \\
&$t^{b}_{28} $  & average max mouseover rank per query. \\
&$t^{b}_{29} $  & total scroll distance in session. \\
&$t^{b}_{30} $  & average scroll distance per query. \\
&$t^{b}_{31} $  & max scroll position in session. \\
&$t^{b}_{32} $  & average max scroll position per query. \\
 &$t^{d}_{1} $  & Number of distinct domains of the visited pages. \\
%& $t^{d}_{2},t^{d}_{3},t^{d}_{4} $  & Maximum, minimum, average pagerank of visited pages. \\
& $t^{d}_{2},t^{d}_{3},t^{d}_{4},t^{d}_{5}$  & Total, maximum, minimum, average page title length. \\
& $t^{d}_{6},t^{d}_{7},t^{d}_{8},t^{d}_{9}$  & Total, maximum, minimum, average page size. \\
\bottomrule 
%\multicolumn{3}{l}{$\dagger$-features extracted based on clustering result}
\end{tabular}
\end{adjustbox}
\label{tab:features}
\end{table}

